From Pixels to Progress: Generating Road Network from Satellite Imagery for Socioeconomic Insights in Impoverished Areas

The Sustainable Development Goals (SDGs) aim to resolve societal challenges, such as eradicating poverty and improving the lives of vulnerable populations in impoverished areas. Those areas rely on road infrastructure construction to promote accessibility and economic development. Although publicly available data like OpenStreetMap is available to monitor road status, data completeness in impoverished areas is limited. Meanwhile, the development of deep learning techniques and satellite imagery shows excellent potential for earth monitoring. To tackle the challenge of road network assessment in impoverished areas, we develop a systematic road extraction framework combining an encoder-decoder architecture and morphological operations on satellite imagery, offering an integrated workflow for interdisciplinary researchers. Extensive experiments of road network extraction on real-world data in impoverished regions achieve a 42.7% enhancement in the F1-score over the baseline methods and reconstruct about 80% of the actual roads. We also propose a comprehensive road network dataset covering approximately 794,178 km2 area and 17.048 million people in 382 impoverished counties in China. The generated dataset is further utilized to conduct socioeconomic analysis in impoverished counties, showing that road network construction positively impacts regional economic development. The technical appendix, code, and generated dataset can be found at https://github.com/tsinghua-fib-lab/Road_network_extraction_impoverished_counties.

==> RelatedWork2.tex <==
\section{Related Work}
\subsection{Satellite Imagery-based Road Extraction}
%The extraction of road networks serves as a fundamental and crucial module in various fields, such as navigation \cite{wang2023hd} and urban computing \cite{lobsang2019can,boeing2022street}. 
With the development of deep learning, satellite imagery has been utilized for road extraction. Mnih~\emph{et al.}~\cite{mnih2010learning} utilize CNN with encoder-decoder architecture to detect roads in high-resolution satellite images. Zhang~\emph{et al.}~\cite{zhang2018road} apply a deep residual U-Net to segment roads in order to optimize the training procedure.
%Panboonyuen~\emph{et al.}~\cite{cheng2017automatic} propose to apply landscape metrics and conditional random fields on CNN to remove the falsely detected road objects. To mitigate the effects of complex backgrounds and occlusions of trees and cars, Cheng~\emph{et al.}~\cite{cheng2017automatic} introduces a cascaded end-to-end convolutional neural network to detect the roads and extract the centerlines at the same time. 
To overcome the road occlusions caused by surroundings, Yang~\emph{et al.}~\cite{yang2022road} introduce RCFSNet, including a multiscale context extraction module and a full-stage feature fusion module to enhance the road area's segmentation quality. To guarantee the connectivity of roads, Wegner~\emph{et al.}~\cite{wegner2015road} adopt the shortest path method as post-processing step to improve the segmentation results. Liu~\emph{et al.}~\cite{liu2018roadnet} further combine the edges and centerlines of roads for better connected segmentation. Mei~\emph{et al.}~\cite{mei2021coanet} propose skip concolution module and connectivity attention module to further guarentee the connectivity of roads as well as romove the effects of occlusions. Those works only consider extracting road masks in limited satellite imagery, and neglect to extract the large-scale road network in impoverished areas for practical socioeconomic analysis.
% There are commonly used training dataset such as the DeepGlobe~\cite{demir2018deepglobe}, SpaceNet~\cite{van2018spacenet}, Massachusetts road dataset \cite{mnih2013machine}, and LoveDA \cite{} for the training and validation of above-mentioned models. 

%The fully-convolutional network (FCN) architecture has shown effectiveness in semantic segmentation of images \cite{long2015fully}.

\subsection{Transportation Infrastructure-based Socioeconomic Study}
Many scholars have explored the effect of transportation infrastructure on economic development on large scales like country or state. Ighodaro~\emph{et al.}~\cite{ighodaro2009transport} study the economic impact of transportation on country level.
%and finds that the lagged value of the road development variable holds substantial importance in influencing the economic growth in Nigeria in the long run. Hong~\emph{et al.}~\cite{hong2011transport} proposes a multi-dimensional measurement transport infrastructure and analyze the linkage between the transportation and economy on the province level in China. 
%Jiwattanakulpaisarn~\emph{et al.}~\cite{jiwattanakulpaisarn2012marginal} investigate the impact of highway capacity expansions on regional economic development at the state level. 
Pradhan~\emph{et al.}~\cite{pradhan2013effect} delve into the impact of transportation infrastructure on the economic growth of India and reveals an unidirectional causality from rail transportation to economic growth. 
%Achour~\emph{et al.}~\cite{achour2016investigating} explore the causal connections between transportation infrastructure and gross capital formation in Tunisia. 
Zhang~\emph{et al.}~\cite{Zhang2023role1} study the relationship between transport infrastructure development and economic growth in the UK. Banerjee~\emph{et al.}~\cite{banerjee2020road} assess the impact of access to transportation networks on regional demographic and economic outcomes in China. At a smaller scale, such as city, the transportation network especially the road network's relationship with socioeconomic activities are studied. Porta~\emph{et al.}~\cite{porta2009street} study the correlation between road network centrality and economic activities. Spadon~\emph{et al.}~\cite{spadon2018topological} utilize the road network topological features to predict demography. Zhou~\emph{et al.}~\cite{zhou2022road} develop a theoretical framework illustrating how road construction facilitates both economic growth and poverty alleviation using panel data. However, the research on road network's socioeconomic impact in impoverished area is still scarse. 

Our work offers a road network extraction framework and corresponding generated dataset for this missing research area, providing relevant researchers and policymakers further help in supporting impoverished counties. 
% Ighodaro~\emph{et al.}~\cite{ighodaro2009transport}
% Ighodaro~\emph{et al.}~\cite{ighodaro2009transport}
